Probing the Efficacy of Federated Parameter-Efficient Fine-Tuning of Vision Transformers for Medical Image Classification

With the advent of large pre-trained transformer models, fine-tuning these models for various downstream tasks is a critical problem. Paucity of training data, the existence of data silos, and stringent privacy constraints exacerbate this fine-tuning problem in the medical imaging domain, creating a strong need for algorithms that enable collaborative fine-tuning of pre-trained models. Moreover, the large size of these models necessitates the use of parameter-efficient fine-tuning (PEFT) to reduce the communication burden in federated learning. In this work, we systematically investigate various federated PEFT strategies for adapting a Vision Transformer (ViT) model (pre-trained on a large natural image dataset) for medical image classification. Apart from evaluating known PEFT techniques, we introduce new federated variants of PEFT algorithms such as visual prompt tuning (VPT), low-rank decomposition of visual prompts, stochastic block attention fine-tuning, and hybrid PEFT methods like low-rank adaptation (LoRA)+VPT. Moreover, we perform a thorough empirical analysis to identify the optimal PEFT method for the federated setting and understand the impact of data distribution on federated PEFT, especially for out-of-domain (OOD) and non-IID data. The key insight of this study is that while most federated PEFT methods work well for in-domain transfer, there is a substantial accuracy vs. efficiency trade-off when dealing with OOD and non-IID scenarios, which is commonly the case in medical imaging. Specifically, every order of magnitude reduction in fine-tuned/exchanged parameters can lead to a 4% drop in accuracy. Thus, the initial model choice is crucial for federated PEFT. It is preferable to use medical foundation models learned from in-domain medical image data (if available) rather than general vision models.

==> Figures_Code_Main_Paper/fine_tune_5_clients.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.7\textwidth]{figures/finetuning_fig2.pdf}
\caption{Performance of different federated PEFT methods. \textbf{Left:} in-domain. \textbf{Right:} out-of-domain. For a fair comparison, we exclude client $4$ from the framework. The performance variability is less pronounced in the in-domain scenario. \textit{LP: linear probing.}}
\label{fig:finetuningfig}
\end{figure}

==> Figures_Code_Main_Paper/intermediate_blocks.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.8\textwidth]{figures/fig_three_blocks_subplot.pdf}
\caption{\textbf{Left:} The performance of federating one single attention block in a vision transformer. \textbf{Right:} Federating different sets of attention blocks. Overall, middle attention blocks demonstrated higher performance.}
\label{fig:blocks_subplots}
\end{figure*}
